InterBERT: Vision-and-Language Interaction for Multi-modal Pretraining

Multi-modal pretraining for learning high-level multi-modal representation is a further step towards deep learning and artificial intelligence. In this work, we propose a novel model, namely InterBERT (BERT for Interaction), which is the first model of our series of multimodal pretraining methods M6 (MultiModality-to-MultiModality Multitask Mega-transformer). The model owns strong capability of modeling interaction between the information flows of different modalities. The single-stream interaction module is capable of effectively processing information of multiple modalilties, and the two-stream module on top preserves the independence of each modality to avoid performance downgrade in single-modal tasks. We pretrain the model with three pretraining tasks, including masked segment modeling (MSM), masked region modeling (MRM) and image-text matching (ITM); and finetune the model on a series of vision-and-language downstream tasks. Experimental results demonstrate that InterBERT outperforms a series of strong baselines, including the most recent multi-modal pretraining methods, and the analysis shows that MSM and MRM are effective for pretraining and our method can achieve performances comparable to BERT in single-modal tasks. Besides, we propose a large-scale dataset for multi-modal pretraining in Chinese, and we develop the Chinese InterBERT which is the first Chinese multi-modal pretrained model. We pretrain the Chinese InterBERT on our proposed dataset of 3.1M image-text pairs from the mobile Taobao, the largest Chinese e-commerce platform. We finetune the model for text-based image retrieval, and recently we deployed the model online for topic-based recommendation.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> content/4_deployment.tex <==
\section{Deployment}
\label{sec:deployment}

% \begin{table}
%     \caption{Data statistics of the dataset TaoMultimodal for the pretraining of the Chinese \interbert.}
%     \label{tab:pretrain_dataset}
%     \begin{tabular}{ccc}
%       \toprule
%           Datasets&Training&Validation\\
%           \midrule
%           Pretraining & 3.1M & 1K\\
%           Finetuning & 200K & 1K \\
%       \bottomrule
%     \end{tabular}
%   \end{table}

\begin{table}[tb]
  \caption{The online results of the deployment of \interbert~and the baseline.}
  \label{tab:ablation}
  \centering
  \begin{tabular}{ccc}
    \toprule
    Model & CTR & Cate. Width \\
        \midrule
       Baseline & 2.32 & 3.45   \\
       InterBERT & 2.51 & 3.48 \\
        % Two-stage & 70.3  \\
        % Out+In & MSM+MRM & - \\
        % Out+In+VCR & MSM+MRM & - \\
    \bottomrule
  \end{tabular}
\end{table}

Besides proposing a novel approach for multi-modal pretraining, we develop the first Chinese multi-modal pretrained model, Chinese \interbert. The model is pretrained on the extracted dataset from the largest Chinese e-commerce platform, the mobile Taobao. 
We extract the representation vector from the pretrained model for each product in the platform, and then apply them directly for item-to-item retrieval to the online recommender system to evaluate its performance in online recommendation.
% Then we finetune the pretrained model on a relatively small dataset of a specific category. The downstream task for finetuning is image-text retrieval, which evaluates the transferability of the pretrained model. 

% \subsection{Experimental Setup}
\vpara{Pretraining} We pretrain our Chinese InterBERT on the extracted data from the mobile Taobao. The pretraining dataset consists of over 100M items, each of which consists of a product image and a product title. 
For preprocessing, we obtain object representations of $2048$ dimensions with an object detector based on Faster-RCNN trained on the data of the mobile Taobao, where there are $33$ categories for object classification. 
% We extract the bounding boxes with confidence scores larger than $0.1$, and we obtain no more than $16$ objects for each image.\footnote{Unlike the other datasets, the images in TaoMultimodal contain relatively fewer objects.} The size of the object representations is $2048$. 
% As to the data cleaning for text, 
We then remove the titles without any Chinese character and those that trigger our spam detector, including texts that are concerned with pornography, abuse, terrorism, etc. 
% Finally, we obtain a dataset of 3.1M image-text pairs for pretraining and 200K for finetuning. 
For release, we build a relatively small dataset of 3.1M product image-text pairs.\footnote{We will soon release the dataset for the research community.} 
% Each pair of data consists of an image of a product and its product title. 
% The products are under the category ``women clothes''. This design is concerned with the evaluation of the pretrained model's transferability to other domains.
% The image demonstrates the key features of the product, and thus they have many fewer objects compared with those of CC and SBU. 
We demonstrate two examples of image-text pair on Figure~\ref{fig:example_taobao}. 
% More details are referred to Appendix~\ref{sec:appendix}. 
% The products cover a wide range of product categories, such as clothes, electronic devices, toys, etc. 
% We preprocess the data and transform them to object sequences.
% We pretrain our \interbert~on the dataset for multi-modal representations. The implementaion details are provided in Appendix~\ref{sec:appendix_impl}.


\vpara{Application to Recommender System}
We further deploy our pretrained model on the recommender system of the mobile Taobao. We extract the multimodal representation for each item with our pretrained Chinese InterBERT (e.g. the representation vector at the ``$[CLS]$'' position). We store the representations and use the offline vector-based KNN service for nearest neighborhood search. For each trigger item, we extract the most relevant $k$\footnote{We empirically use $5$ based on our preliminary online experiments.} items with the KNN service. The online service receives the triggers from user histories and searches the relevant items, whose query latency is around 10ms. A separate ranking system is responsible for the final results to the users. We compare our method with a single-modal BERT-based model.\footnote{Here we only compare with the content-based baseline, instead of the collaborative filtering methods.} Specifically, we extract the text embeddings of product titles with a Chinese BERT further pretrained on the data of the mobile Taobao, and then apply the above-mentioned process. 
For the online A/B testing, we provide each method with at least 5\% traffic and observe each trail for at least 7 days.
% We finetune our Chinese \interbert~on the other of our extracted dataset of image-text pairs from the mobile Taobao. The process of dataset construction is similar to that of the pretraining data. The dataset contains around 200K image-text pairs, which belong to the products under the category ``women shoes''. The finetuning of the Chinese \interbert~is designed for a downstream task, text-based image retrieval. 
% Given a piece of text, the model should retrieve the images that are related to the text from the given pool. 
% This task evaluates the model's ability of image retrieval based on the given linguistic information and the model's transferability to a specific category. 
% We test the model on a test set of around 22K texts, each of which has a pool of images for retrieval. 
% Furthermore, recently we have deployed the model online for the topic-based recommendation for women shoes. More details are referred to Appendix~\ref{sec:appendix_deploy}. 
% In the online context, the model recalls the relevant products by recalling images related to a given topic (usually a phrase or a sentence) and creates a topic-based bundle for recommendation. 


% \vpara{Implementation Details}
% We apply the same setting of the English \interbert~to the pretraining and finetuning of the Chinese \interbert.

\vpara{Results} We observe the click-through rates of the trails of the retrieval of multimodal representation and that of text representation. On average, the multimodal retrieval outperforms the competitor by around $+8.2\%$ (2.51 vs 2.32). This demonstrates that the similarity search based on multimodality is more consistent with the user interests than the one based on plain text. Also, we report the exposed category width, which refers to the average number of exposed categories in a browsing session. Our model has an advantage of $+0.9\%$ over the baseline (3.48 vs 3.45), which shows that the multimodal retrieval brings more diversity to the user experience through visual and linguistic similarity.


% 这个在考虑改成figure，折线图的样式，说明预训练在下游数据越少的情况下表现越突出
% \begin{table}
%     \caption{Data statistics of the dataset TaoMultimodal for the pretraining of the Chinese \interbert. The evaluation metrics are P@1, P@5 and P@10.}
%     \label{tab:chinese_result}
%     \begin{tabular}{cccc}
%       \toprule
%           Model & P@1 & P@5 & P@10\\
%           \midrule
%           \interbert & 57.0 & 57.2 & 56.9\\
%           w/o pretraining & 51.8 & 54.5 & 55.2\\
%       \bottomrule
%     \end{tabular}
%   \end{table}
% The click-through rate of the model surpasses that of the conventional text-to-text retrieval by 1.1\%.

% \begin{figure}
%     \centering
%     % \begin{minipage}{.22\textwidth}
%         \centering
%         \begin{tikzpicture}
%         \selectcolormodel{RGB}
%         \begin{axis}[legend pos=north west, ylabel={P@5}, ybar, enlargelimits=0.25, bar width=5.2mm, symbolic x coords={10K, 100K, 200K}, nodes near coords,
%             nodes near coords align={vertical},ymin=33.0, ymax=64.3]
%         \addlegendentry{w/o prt}
%         \addplot 
%         coordinates{(10K, 29.9)(100K, 54.5)(200K, 64.3)};
%         % \legend{Seq2Seq}
        
%         \addlegendentry{prt}
%         \addplot 
%         coordinates{(10K, 33.5)(100K, 57.2)(200K, 64.9)};
        
%         % \legend{ACA}
%         \end{axis}
%         \end{tikzpicture}
%     \caption{Results (P@5) of the models with and without pretraining in the text-based image retrieval task. ``prt'' refers to pretraining. The models are finetuned on datasets of different sizes, including 10K, 100K and 200K. Experimental results show that pretraining is more effective when there are fewer data for finetuning.}
%     \label{fig:taobao_result}
%     \end{figure}
